Distance Preserving Graph Simplification

Large graphs are difficult to represent, visualize, and understand. In this paper, we introduce "gate graph" - a new approach to perform graph simplification. A gate graph provides a simplified topological view of the original graph. Specifically, we construct a gate graph from a large graph so that for any "non-local" vertex pair (distance higher than some threshold) in the original graph, their shortest-path distance can be recovered by consecutive "local" walks through the gate vertices in the gate graph. We perform a theoretical investigation on the gate-vertex set discovery problem. We characterize its computational complexity and reveal the upper bound of minimum gate-vertex set using VC-dimension theory. We propose an efficient mining algorithm to discover a gate-vertex set with guaranteed logarithmic bound. We further present a fast technique for pruning redundant edges in a gate graph. The detailed experimental results using both real and synthetic graphs demonstrate the effectiveness and efficiency of our approach.

==> Alg.tex <==
\section{Our Algorithms}
\label{algorihm}

In this section, we first analyze the problem and introduce an interesting property of $\epsilon-neighbors$ which can guarantee the satisfactory of second condition in graph simplification problem.
Afterward, we formulate the {\em Gates Discovery Problem} to be an instance of set cover problem based on this property.
Given those gates, an efficient approach is proposed to generate the minimal number of edges to connect the gates.


\subsection{Algorithm for Gates Discovery Problem}
\label{gatealg}

In this work, we focus on the shortest distance no less than $\epsilon$, as the local distance can be efficiently achieved provided that $\epsilon$ is a small constant.
That is, if one vertex is contained in the $\epsilon-neighbors$ of another vertex, their shortest distance is allowed to be online computed.
In addition, the shortest distance in graphs is a metric which holds the triangle inequality.
Therefore, given source $u$, destination $v$ and vertex $x$, if $x$ belongs to shortest path $SP_{u,v}$, then both segment $P_{u,x}$ and $P_{x,v}$ are shortest paths.
In other words, $d_G(u,v)= d_G(u,x) + d_G(x,v)$.
Then, we have the following observation:

\bobserv
Let $u$, $v$, $x$ and $y$ be the vertices of graph $G$, and $x$ and $y$ are distinct from $u$ and $v$.
If there exits a shortest path $SP_{u,v}$ contains $x$ and $y$, then the subpath $P_{x,y} \subset SP_{u,v}$ is the shortest path (i.e., $d_G(u,v) = d_G(u,x) + d_G(x,y)+d_G(y,v)$).
\eobserv

Recall the procedure of computing shortest distance based on $\epsilon-neighbors$ and simplified graph,
we have to find out the appropriate gates $x$ and $y$ which are contained in the source and destination's $\epsilon-neighbors$, respectively.
How to find the smallest number of such vertices is also the goal of {\em Gates Discovery Problem}.
Interestingly, for each vertex $u$ in the graph, we observe that if we can identify a subset of vertices from $\epsilon-neighbors$ as its {\em gates} which can lead to the vertices $v^\prime$ where their distances $d_G(u,v^\prime)$ is $\epsilon+1$,
we can restore the distance from $u$ to any its reachable vertex $v$.

Before we formally summarize the above property, we first introduce the definition of {\em coverage} in terms of shortest distances:

\comment{
\bdefin
Let $u$, $v$ and $x$ be the vertices of graph $G$.
If $x$ lies in one of the shortest path $SP_{u,v}$ between $u$ and $v$ (i.e., $d_G(u,v) = d_G(u,x)+d_G(x,v)$),
then we say $x$ covers the shortest distance between $u$ and $v$.
\edefin
}

\bdefin{\bf (Vertex Coverage)}
\label{vcdef}
Let $L$ be a set of vertices and $S = \{(u_0,v_0), ..., (u_k, v_k)\}$ be a set of vertex pairs in the graph $G$.
We say that $L$ covers $S$ if for each vertex pair $(u_i,v_i)$ there is at least one vertex $x \in L$ such that $d_G(u_i,v_i)=d_G(u_i,x) + d_G(x,v_i)$.
\edefin

Given this, we observe the following property:

\blemma{\bf (Shortest Distance Restoration Property)}
\label{restorelemma}
For each vertex $x$ in the graph $G$, if a subset of vertices $L(x) \in \epsilon-neighbors(x)$ can cover all vertex pairs $\{(x,y_i)\}$ where $d_G(x,y_i) = \epsilon+1$,
then we are able to compute the shortest distance between any pair of vertices $u$ and $v$ by:
\[ d_G(u,v) = min_{x \in L(u) \wedge y \in L(v)} (d_G(u,x) + d_G(x,y) + d_G(y,v)) \]
\elemma


\bproof
We focus on the shortest distance no less than $\epsilon+1$.
For any shortest path $P=(v_1,...,v_k)$ with the length $k > \epsilon$, it contains the shortest path $SP_1=(v_1,...,v_{\epsilon})$ and $SP_2=(v_{k-\epsilon+1}, ..., v_k)$.
Since we have guaranteed that one vertex $x_0 \in L(v_1)$ lies in the path $SP_1$ and one vertex $y_0 \in L(v_k)$ belongs to the path $SP_2$,
we have two vertices $x_0$ and $y_0$ in the shortest path $P$.
Now, we consider the shortest path between $x_0$ and $y_0$.
Its shortest distance has two cases: 1) $d_G(x_0,y_0) \le \epsilon$; or 2) $d_G(x_0,y_0) > \epsilon+1$.

\noindent{Case 1:} $x_0$ and $y_0$ are each other's $\epsilon-neighbors$, thus the shortest distance can be calculated directly.
Then, we compute the shortest distance by concatenating three shortest distances as follows:
\[ d_G(v_1,v_k) = d_G(v_1, x_0) + d_{G}(x_0,y_0) + d_G(y_0,v_k) \]

\noindent{Case 2:} following similar idea, we always have one vertex $x_1 \in L(x_0)$ and one vertex $y_1 \in L(y_0)$ belonging to shortest path $SP_{x_0,y_0}$.
In this way, we convert the problem of computing shortest distance $x_0$ and $y_0$ to computing the distance between $x_1$ and $y_1$.
Since both $x_1$ and $y_1$ lie in the shortest path $SP_{x_0,y_0}$, we make sure that $x_1$ and $y_1$ also belong to shortest path $SP_{u,v}$ and always have $d_G(x_0,y_0) = d_G(x_0,x_1) + d(y_1, y_0)$.
We recursively find $x_{i+1} \in L(x_i)$ and $y_{i+1} \in L(y_i)$ that lie in the shortest path $SP_{u,v}$ (case 2) until the distance $d_G(x_m,y_m) \le \epsilon$ (case 1).
That is, the distance between $x_i$ and $y_i$ can be formulated as a recursive expression:
$d_G(x_i,y_i) = d_G(x_i,x_{i+1}) + d_G(x_{i+1},y_{i+1}), d_G(y_{i+1}, y_i)$ if $d_G(x_{i+1},y_{i+1})\ge \epsilon$.
Given this, we concatenate all shortest distances through $x_i$ and $y_i$ to compute $d_G(u,v)$ as follows:
\beqnarr
 d_G(v_1,v_k) = d_G(v_1, x_0) + \sum_{i=1}^m d_G(x_{i-1},x_i) +  d_{G}(x_m,y_m) \nonumber \\
        + \sum_{i=1}^m d_G(y_{i-1},y_i) + d_G(y_0,v_k) \nonumber
\eeqnarr
where $d_G(x_m,y_m)$ has been demonstrated in case 1.
\eproof


Clearly, the goal of our {\em Gates Discovery Problem} is to minimize $|\cup_{v \in V} L(v)|$.
We transform the problem to an instance of cardinality set cover problem.
{\em Let $S=\{(x,y)\}$ be the ground set to be covered, where $d_G(x,y) = \epsilon+1$.
For each vertex $u$ in the graph, it is associated with a set of vertex pairs $S_u \subseteq S$, where each pair $(x,y) \in S_u$ holds the condition $d_G(x,y)=d_G(x,u)+d_G(u,y)$.
Further, we assign the unit cost to each vertex in the graph, i.e, $cost(u) = 1$.
Given this, our {\em Gates Discovery Problem} is converted to the problem of seeking a subset of vertices $V^\ast \in V$ to cover the ground set,
i.e., $S = \cup_v S_v$, with the minimal cost $\sum_v cost(v)$.}
As we know, the set cover problem is NP-hard, and a greedy algorithm with logarithmic approximation ratio exits.
The traditional greedy algorithm works as follows: {\em for each iteration, we always select one set which maximally covers the remaining uncovered elements until all elements in the ground set are covered.}
The algorithm tries to make the ``best'' choice at each iteration which leads to a reasonable ``good'' solution globally.

In order to adopt greedy algorithm for discovering gates, we first have to generate the ground set $S$ and each candidate subset $S_x$ associating with vertex $x$.
In other words, all shortest paths with length $\epsilon+1$ are required, such that two endpoints of each shortest path is put into ground set and all intermediate vertices lying in the shortest path are used to constitute candidate subsets.
An straightforward solution is to precompute distances of all pairs of vertices with distance no greater than $\epsilon+1$, then for each pair of vertices $(u,v)$,
we check whether vertex $x$ lie in shortest path by comparing the sum of distance between $u$ and $x$, and distance between $x$ and $v$ with $\epsilon+1$.
For large unweighted graphs, the computational cost of distance computation by employing several rounds of breath-first-search (BFS) and intermediate vertices checking is rather expensive, and it is also overwhelming to store entire distance matrix in the memory.

Here, we introduce a procedure which adopts BFS only one time for each vertex to collect all information we need for set cover problem.
Let us the shortest paths from vertex $u$ if $\epsilon=2$ is provided (as shown in Figure \ref{bfsexample}).
In Figure \ref{fig:bfs}, $u$ and its $(\epsilon+1)-neighbors$ are organized from the perspective of breath-first-search (i.e., in terms of visiting levels).
The black line represents the BFS visiting path (e.g., $(u,x_1)$ means visiting $x_1$ from $u$),
the blue line represents the interconnections within the same level (e.g., $(x_1,x_2)$), and red line represent the connections between two visited vertices in different levels (e.g., $(x_2,v_2)$ where $v_2$ has been checked by $x_1$ when $x_2$ is considered).
Any vertex in this structure only has those 3 types of connections.
Remind that our goal is to collect all immediate vertex within the shortest paths from $u$ to $v_5$ in this example.
For each vertex $v$, if its immediate neighbors in the lower level can record those immediate vertices from $u$ to them, all intermediate vertices reach $v$ through shortest paths from $u$ can be obtained by the union of all its lower-level neighbors' sets.
Since two vertices in the same level do not provide more information for each other, they are omitted here.

\begin{figure}
    \centering
    \mbox{
        \subfigure[Example for Algorithm \ref{alg:bfssetcover}] {\epsfig{figure=Figures/BFSSetCover.eps,scale=0.6} \label{fig:bfs}}
        \subfigure[Example for Set Cover]{\epsfig{figure=Figures/setcoversetting.eps,scale=0.6}\label{fig:setcover}}
    }
    \label{bfsexample}
    \caption{Example for Gate Discovery Algorithm ($\epsilon=2$)}
\end{figure}


In the example (following the procedure outlined in Algorithm \ref{lg:bfssetcover}), we start from $u$ to visit its neighbors $x_1$, $x_2$ and $x_3$.
All currently visited neighbors $x_i$ are put into a queue and their associated set $P(x_i)$ are updated in the meanwhile.
Likewise, $v_1$ and $v_2$ are visited and push into queue when $x_1$ is popped from the queue.
When $x_2$ is popped, we consider all its neighbors $x_1$, $v_2$ and $v_4$ in 3 different cases:
{\em
1) $x_1$ has been visited and in the same level with $x_2$, we omit it as no information is provided;
2) $v_2$ has been visited and in the higher level, we need to update its associated set by combining the intermediate vertices in $P(x_2)$ (Line 13 to Line 15);
3) $v_4$ is currently visited, so its associated set $P(v_4)$ is initialized by $P(x_2) \cup \{x_2\}$.
}
The procedure repeats until all vertices in the $(\epsilon+1)-neighbors$ are processed.
According to their associated sets, we can generated the ground set and each vertex's associated subset for set cover problem as illustrated in Figure \ref{fig:setcover}.



\input{Figures/BFSSetCover.tex}

\comment{
\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/BFSSetCover.eps,scale=0.6}
\end {tabular}
\caption {Illustrative Example for Algorithm \ref{alg:bfssetcover}}
\label{bfsexample}
\end{figure}
}


The entire algorithm for gate discovery includes two key steps:

\noindent{\bf 1. Set-Cover Initialization: }

For each vertex $u$, we call procedure $BFSSetCover$ to generate vertex pairs with distance $\epsilon+1$ and all intermediate vertices lying in the shortest paths.
We repeat the procedure $|V|$ times to complete the initialization of set-cover setting.

\noindent{\bf 2. Greedy Gate Discovery: }

In each iteration, we select one vertex $v$ which associates largest number of uncovered vertex pairs with distance $\epsilon+1$.
The procedure proceeds until all vertex pairs in the ground set are covered.


\comment{
\input{Figures/GatesDiscovery.tex}

The overall procedure to discover gate is outlined in Algorithm \ref{alg:gatesdiscovery}.
We use $V^\ast$ to store the resulting {\em gates}, and $R$ to record the set of the set of vertex pairs which has been covered during the procedure.
The procedure starts with initializing $V\ast$ and $R$ to be empty set (Line 1 and Line 2).
Then, breath-first-search (BFS) traversal is employed $|V|$ times to gain all vertex pairs whose shortest distance is $\epsilon+1$.
During the procedure of BFS, the ground set $S$ recording all vertex pairs with distance $\epsilon+1$ is collected,
and each vertex $v$'s associated set $S_v$ is also updated (Line 3 to Line 5).
In the while loop for greedy cover (Line 6 to Line 10), for each iteration, we always choose an unselected vertex $v$ such that $\frac{1}{S_v \cap (S \setminus R)}$ is minimum (Line 7).
In the meanwhile, $V^\ast$ and $R$ are also updated (Line 8 to Line 9).
This procedure repeats until all vertex pairs are covered in $R$ and the resulting gates are stored in $V^\ast$.
}

\noindent{\bf Complexity:}
The first step for collecting ground set and each vertex's associated set takes $O(|V|(|V|+|E|))$ since $|V|$ times BFS are employed and each BFS takes $O(|V|+|E|)$ time.
For the implementation of greedy set cover procedure, utilizing the speedup queue technique which have mentioned in \cite{Schenkel04,DBLP:conf/sigmod/JinXRF09},
assuming we only need to visit $d \ll |V|$ vertices in the queue (i.e., all vertices are ranked in ascending order in the queue),
each step takes $O(d(\log |V| + 1))$ time to exact and update the queue.
As greedy procedure has $O(|V^\ast|)$ steps, it takes $O(d |V^\ast| (\log |V| +1))$ in total.
Putting both together, this algorithm's time complexity is $O(d |V^\ast| \log |V|  + |V| |E|)$.

\noindent{\bf Speeding up the greedy algorithm:}
A potential issue of our gate discovery algorithm is that it requires materialization of the vertex pairs whose distance is no greater than $\epsilon+1$ (i.e., ground set),
which is needed for greedy set cover procedure.
If graph diameter is very close to $\epsilon$, the size of vertex pairs can be very close to the size of transitive closure, which is hard to be hold in the main memory.
To handle large graphs, we adopt partial set cover strategy.
Instead of trying to cover all the shortest pairs with distance $\epsilon+1$, we first pick a set of vertices $V^\ast_b$ with high betweenness as our gates.
The vertex betweenness based on the shortest path no longer than $\epsilon$ can be easily estimated during BFS traversal.
This actually follows the basic idea of greedy set cover procedure, because the vertex with high betweenness tends to cover more shortest pairs in the greedy procedure.
Then, only the vertex pairs which have not covered by $V^\ast_b$ are considered in the set cover framework.
Supposing a large portion of vertex pairs are covered by the vertex with high betweenness, the size of ground set in set cover framework would be significantly reduced,
which eventually avoids the memory bottleneck.

\bthm
Gate Discovery Algorithm achieves $\ln K$ approximation ratio with respect to the optimal solution,
where $K$ is the number of vertex pairs whose shortest distance is $\epsilon+1$.
\ethm

\input{EdgeSparsification.tex}


\comment{
\subsection{Algorithm for Edge Discovery Problem}
\label{edgealg}

In this subsection, we study the problem: {\em how to find minimal number of edges to connect the discovered gates while maintaining the property of distance restoration?}
Recall that the shortest distance between any two gates can be restored only using other gates that belongs to their $\epsilon-neighbors$.
This is because the gates are a subset of vertices in the original graph and lemma \ref{restorelemma} is also applicable here.
To explicitly visualize the connectivities among gates, we introduce the concept of {\em Gate Graph} and {\em $k$-hop neighbors} as follows:

\bdefin{\bf (Gate Graph)}
\label{gategraph}
Let $G=(V,E)$ be graph, its discovered gates $V^\ast$ and parameter $\epsilon$.
The weighted graph $G^\prime=(V^\ast, E^\prime,W)$ is gate graph if and only if there is a edge between a pair of gates $u$ and $v$ where $d_G(u,v) \le \epsilon$, and $w(u,v)=d_G(u,v)$.
\edefin

\bdefin{\bf ($k$-hop Neighbors)}
\label{hopneighbor}
Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
In the gate graph, we say vertex $v$ is vertex $u$'s $k$-hop neighbor if and only if there is a shortest path between $u$ and $v$ with $k$ edges in $G^\prime$.
\edefin

In the gate graph, sufficient relationships for computing shortest distance, such as $\epsilon-neighbors$, are preserved, thus all shortest distances of any pair of vertices are maintained.
However, we will see that some edges in the gate graph are not necessary which can be removed without affecting the computation of shortest distance.
On the other hand, the {\em Edge Discovery Problem} aims to find minimal number of edges connecting {\em gates} while preserving the properties.
Fortunately, there is interesting connection between the result of {\em Edge Discovery Problem} and gate graph:
the resulting edges belongs to the edge set of gate graph.

\blemma
\label{edgelemma}
Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
The Edge Discovery Problem on graph $G$ is equivalent to the problem of extracting minimal number of edges from gate graph which holds the following property:
\beqnarr
 d_G(u,v)=  \nonumber \\
 min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon} ( d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v) )  \nonumber
\eeqnarr
\elemma
}

\comment{
\bproof
Let us first assume that the result of Edge Discovery Problem is edge set $E^\ast$.
In the proof, we want to show that $E^\ast$ is the subset of edge set $E^\prime$ in the gate graph.
According to lemma \ref{restorelemma}, for any pair of vertices, there exits a set of gates lying in one of its shortest path, where the distance between two neighboring gates are no greater than $\epsilon$.
Otherwise, at least one vertex pair's shortest distance cannot be restored.
In addition, gates are also a subset of vertices in the original graph, thus each gate also has to connect some other gates within its $\epsilon-neighbors$ to cover all shortest distances to $(\epsilon+1)-neighbors$ in the original graph.
According to our problem definition, we easily see that the distance between one gate with its 2-hop neighbors are greater than $\epsilon$ in the gate graph.
That is, each gate need to connect to some immediate neighbors (i.e., 1-hop neighbors) in order to maintain distance restoration property.
This also means, for each gate, some of its immediate neighbors are redundant.
Thus, the result of Edge Discovery Problem $E^\ast$ is the subset of edges of gate graph $G^\prime$.
\eproof
}

%\bproof
%Let us first assume that the result of Edge Discovery Problem is edge set $E^\ast$.
%In the proof, we want to show that $E^\ast$ is the subset of edge set $E^\prime$ in the gate graph.
%To achieve this, to maintain distance restoration property, we first prove that each gate $v \in V^\ast$ should connect to all its 2-hop neighbors via shortest paths going through $v$'s immediate neighbors.
%Then, we further prove that the above mentioned shortest path actually is an single edge.
%
%According to lemma \ref{restorelemma}, for any pair of vertices, there exits a set of gates lying in one of its shortest path, where the distance between two neighboring gates are no greater than $\epsilon$.
%Otherwise, at least one vertex pair's shortest distance cannot be restored.
%In addition, gates are also a subset of vertices in the original graph, thus each gate also has to connect some other gates within its $\epsilon-neighbors$ to cover all shortest distances to $(\epsilon+1)-neighbors$ in the original graph.
%According to the definition of gate discovery problem, we easily see that the distance between one gate with its 2-hop neighbors are greater than $\epsilon$ in the gate graph.
%Furthermore, for each gate $v$ in the gate graph, there is no guarantee to have $(\epsilon+1)-neighbors$.
%However, if each gate has shortest paths to reach all its 2-hop neighbors, then we are able to compute shortest distance for every pair of gates following similar proof in lemma \ref{restorelemma}.
%Therefore, each gate $v \in V^\ast$ should connect to all its 2-hop neighbors via shortest paths going through $v$'s immediate neighbors.
%
%Given this, we say that there is no gate lying in the shortest path from vertex $u$ to one of its immediate neighbors.
%Considering the original graph, if there is one gate $x$ lying in the shortest path from $u$ to one of its immediate neighbors $v$, we do not need to select $v$ as gate any more.
%This is because shortest distances from vertex $u$ to its $(\epsilon+1)-neighbors$ covered by $v$ can also be covered by vertex $x$, as $d_G(u,v)=d_G(u,x)+d_G(x,v)$.
%
%Recall the edge set of gate graph, it satisfies both conditions and can serve as a feasible solution to retain distance restoration property.
%Thus, the solution of Edge Discovery problem is a subset of edge set in the gate graph.
%%On the other hand, for each vertex, knowing their gates is sufficient to compute all pair of shortest distances as claimed in Lemma \ref{restorelemma}.
%%This means any edge connecting two vertices with distance greater than $\epsilon$ is redundant.
%%Given this, The Edge Discover Problem on graph $G$ can be transformed to the problem of extracting minimal number of edges $E^\ast \in E^\prime$ which holds the property of distance restoration.
%\eproof
%
%
%\begin{figure}
%\centering
%\begin{tabular}{c}
%\psfig{figure=Figures/edgediscovery.eps,scale=0.6}
%\end {tabular}
%\caption {Example for Edge Discovery Problem}
%\label{edgediscoverexample}
%\end{figure}
%
%
%According to lemma \ref{edgelemma}, we transform our edge discovery problem to the problem of finding minimal number of edges from gate graph.
%In addition, following the similar idea of lemma \ref{restorelemma}, in order to hold distance restoration property in the gate graph,
%each gate $u$ should connect to some of its immediate neighbors (i.e., 1-hop neighbors) which cover all shortest distances from $u$ to its 2-hop neighbors.
%Here, we use 1-hop neighbors since gate graph is a weighted graph where each edge weight corresponds to the shortest distance between two connected vertices.
%Also, for each vertex $u$, its immediate neighbors are actually its $\epsilon-neighbros$ since $w(u,v) \le \epsilon$ and $v \in \epsilon-neighbor(u)$,
%and the distance to its 2-hop neighbors are greater than $\epsilon+1$.
%Take figure \ref{edgediscoverexample} as example.
%For vertex $u$, its immediate neighbors are $\{x_1,x_2,x_3,x_4\}$ and 2-hop neighbors are $\{v_1,v_2,...,v_8\}$.
%To hold the property of distance restoration, we can select edge set $\{(u,x_1),(u,x_2),(u,x_3)\}$ or $\{(u,x_1),(u,x_3),(u,x_4)\}$ to cover all 2-hop neighbors.
%
%However, we cannot select the edge set for each vertex individually.
%The central challenge here is original graph is undirected graph and each edge serves as the intermediate edge within different shortest paths from both directions.
%More importantly, the effectiveness of the edge relies on its incident edges, meaning one edge should incorporate with other edges to form the shortest path.
%For instance, in order to use edge $(u,x_1)$ as the edge in the shortest path from $u$ to $v_1$, we have to guarantee that the edge $(x_1,v_1)$ is also chosen.
%Therefore, we cannot directly apply traditional set cover approach to find the minimal number of edges from gate graph.
%Interestingly, we find that our problem can be transformed into a new variant of set cover problem, referred to as {\em Set-Cover-with-Pairs} (SCP) problem.
%
%\bdefin{\bf (Set-Cover-with-Pairs Problem ~\cite{HS05})}
%\label{scpdef}
%Let $U$ be the ground set and let $S = \{1, \ldots, M\}$ be a set of objects, where each object $i\in S$ has a non-negative cost $w_i$. For every $\{i,j\}\subseteq S$, let $\mathcal{C}(i, j)$ be the collection of elements in $U$ covered by the pair $\{i, j\}$. The objective of the set cover with pairs (SCP) problem is to find a subset $S^\prime \subseteq S$ such that
% $\mathcal{C}(S^\prime) =\bigcup_{\{i,j\}\subseteq S^\prime} \mathcal{C}(i, j) = U.$
% with a minimum covering cost $\sum_{i\in S} w_i$.
%We refer to the special case in which each object has  a unit weight ($w_i=1$) as the \textbf{cardinality SCP} problem.
% \edefin
%
%Before we go to the solution, we first define {\em edge coverage} here:
%
%\bdefin{\bf (Edge Coverage)}
%Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
%We have two edges $e_1=(u,x) \in E^\prime$, $e_2=(y,v) \in E^\prime$, and vertex pair $(u,v)$ where $u$ and $v$ are each other's 2-hop neighbor.
%We say $e_1$ and $e_2$ cover vertex pair $(u,v)$ if and only $x$ and $y$ are the same vertex and $d_G(u,v)=w(u,x)+w(y,v)$.
%\edefin
%
%That is, edges $e_1=(u,x)$ and $e_2=(y,v)$ constitutes the shortest path from vertex $u$ to $v$ in the gate graph.
%Given this, we have the ground set $U=\{(u_0,v_0),(u_1,v_1),...\}$ where $u_i$ and $v_i$ are each other's 2-hop neighbor.
%Then, we also have the edge set $E^\prime$ as the object set $S$ where each edge is assigned with unit cost.
%Also, each pair of edge $e_1$ and $e_2$ is associated with single vertex pair $\mathcal{C}(e_1,e_2)$ which can be {\em covered} by them (i.e., $e_1$ and $e_2$ are concatenated to be a shortest path between such pair).
%Our goal is to find a subset of edges $E^\ast \in E^\prime$ such that $\mathcal{C}(E^\ast)=\bigcup_{\{e_i,e_j\}\subseteq E^\ast} \mathcal{C}(e_i, e_j) = U$,
%with minimum cost $|E^\ast|$ (i.e., minimum number of edges within $E^\ast$).
%Since our problem is the instance of SCP problem which has been proven to be NP-hard, we have:
%
%\bthm
%The edge discovery problem on gate graph is NP-hard.
%\ethm
%
%
%\begin{figure}
%    \label{expfig}
%    \centering
%    \mbox{
%        \subfigure[Gate Graph] {\epsfig{figure=Figures/gategraphexample.eps,scale=0.6} \label{fig:gategraph}}
%        \subfigure[Set-Cover-with-Pairs Setting]{\epsfig{figure=Figures/setcoverpairs.eps,scale=0.6}\label{fig:setcoverwithpairs}}
%    }
%    \label{scpexample}
%    \caption{Example for Edge Discovery Algorithm}
%\end{figure}
%
%Let us consider the example in Figure~\ref{scpexample}, where gate graph is shown in Figure~\ref{fig:gategraph}.
%Note that, we omit the edge weight in Figure~\ref{fig:gategraph} for simplification, and the shortest paths including 3 vertices are specified in the lower part.
%As discussed, each shortest path identified by two endpoints is make up of two edges which serve as objects in the traditional Set-Cover-with-Pairs problem (Definition \ref{scpdef}).
%And two endpoints forms a vertex pair included in the ground set.
%According to underlying shortest paths, we visualize the edge-pair covering structure in Figure~\ref{fig:setcoverwithpairs}.
%There is an edge in the covering structure if and only if two edges form a shortest path in the gate graph.
%For instance, there is a shortest path $(v_2,v_8,v_7)$ which is the concatenation of edge $(v_2,v_8)$ and edge $(v_7,v_8)$.
%Therefore, we connect $(v_2,v_8)$ and $(v_7,v_8)$ in the edge-pair covering structure.
%Also, shortest path between $v_2$ and $v_7$ can be covered by edge $(v_2,v_3)$ and $(v_3,v_7)$.

\comment{
\input{Figures/EdgeDiscovery.tex}

Borrowing the idea for solving SCP problem in~\cite{DBLP:conf/fsttcs/HassinS05}, we describe our procedure for edge discovery problem in Algorithm \ref{alg:edgediscovery}.
It begins with initializing the resulting edge set $E^\ast$ and intermediate cover set $R$ to be empty set (Line 1 to Line 2).
For each vertex $u$, we adopt procedure {\em BFS} similar to Algorithm \ref{alg:bfssetcover} to obtain the ground set $U$ and each vertex's associated vertex pairs (Line 3 to Line 5).
In the main while loop (Line 6 to Line 15), for each iteration, we greedily select an edge or an pair of edges which can minimize the cost
$\frac{1}{|\mathcal{C}(E^\ast \cup\{e_i\})\backslash\mathcal{C}(E^\ast)|}$ or $\frac{2}{|\mathcal{C}(E^\ast\cup\{e_i,e_j\})\backslash\mathcal{C}(E^\ast)|}$.
Then, we update the resulting set $E^\ast$ and intermediate cover set $R$ correspondingly (Line 9 to Line 14).
We repeat such iteration until entire ground set $U$ is covered.
Combining the discovered gates $V^\ast$ and the edge set $E^\ast$, the simplified graph $G^\ast$ is returned (Line 16).


\subsubsection{Alternate Greedy Algorithm}
\label{approxgreedy}

Aforementioned greedy algorithm has been proved to have an $O(\sqrt{N \log N})$ approximation ratio, where $N = |U|$ is the size of ground set.
Here, we present an alternate greedy algorithm which considers the potential benefit to evaluate each edge in the selection procedure.
Our greedy algorithm works as follows: {\em each time we select an edge according to our defined criterion, until all elements in the ground set, i.e., all 2-hop vertex pairs in the gate graph, have been covered.}

To describe our edge-selection criterion, we introduce the following definitions:
Let $U$ be the ground set and $R$ be the set recording the already covered vertex: $R \subseteq U$.
Let $S$ be the set of already selected edges and let $\overline{S}$ denote the unused edges in $E^\prime$, $\overline{S}=E^\prime \setminus S$.
Using the graph formulation, we construct a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where each vertex in $\mathcal{V}$ represents one edge in $E^\prime$.
And, there is an edge $(e_x,e_y) \in \mathcal{E}$ if and only $e_x$ and $e_y$ in the gate graph concatenate with each other to form a shortest path from one endpoint of $e_x$ to one endpoint of $e_y$.
In addition, each edge $\mathcal{e} \in \mathcal{E}$ is associated with one vertex pair corresponding to two endpoints of covered shortest path.

Given this, in the graph $\mathcal{G}$, we assume at some iteration, the vertex $v$ is to be selected.
Let $\mathcal{E}(v)$ denotes the set of edges in $\mathcal{G}$ adjacent to $v$.
Then $\mathcal{E}(v)$ covers a set of vertex pairs in $U \setminus R$.
We categorize $\mathcal{E}(v)$ into two parts:
1) one part is immediately covered by selecting $v$;
in other words, $v$ will work directly on those already selected nodes in $S$, denoted as $S_{v}$, to cover this part of the elements;
2) the other part is those elements which may be covered in the future when selecting nodes in $Z_{v}$, where $Z_{v}\subseteq \overline{S}$ and each node in $Z_{v}$ is adjacent to $v$.
It is easy to see $|S_{v}|$ is exactly how many new elements will be covered if we select $v$ at step $i$,
and $|Z_{v}|$ is how many new elements will be {\em potentially} covered as a consequence of selecting $v$.
In other words, $|S_{v}|+|Z_{v}|$ is the upper bound of the number of elements which can be covered by selecting node $v$.
In our algorithm, at each iteration, we select node $v$ from $\overline{S}$ with minimum $\frac{1}{|S_{v}|+|Z_{v}|}$.
Intuitively, we can see that our algorithm with its criteria is ``optimistic'' or ''far-sighted'' as it always selects the node with ``maximal potential'' ($\max {|S_{v}|+|Z_{v}|}$) .
However, the original greedy algorithm~\cite{DBLP:conf/fsttcs/HassinS05} is ``pessimistic''  or ``short-sighted'' as it always selects the node with the immediate best output ($\max {|S_{v}|}= \max {|\mathcal{C}(R\cup\{i\})\backslash\mathcal{C}(R)|}$).
The sketch of new greedy algorithm is outlined in Algorithm~\ref{alg:newedgediscovery}.

\input{Figures/GatesDiscoveryNew.tex}

}

\comment{
\subsection{Greedy Refinement Algorithm}
\label{greedyrefine}

The traditional greedy algorithm for Set-Cover-with-Pairs problem yields $O(\sqrt(N \log N))$ approximation ratio, where $N$ is the number of size of ground set $N = |U|$.
In our problem for edge discovery, the size of ground set is the same with the number of shortest paths containing 2 edges in the gate graph.
In the worst case, $N$ could be very large and the approximation ratio is not attractive enough.
Moreover, as speedup technique with queue for greedy algorithm of set cover problem is not applicable here,
it is very time consuming to choose ``best'' object in each iteration by scanning all remaining objects and checking their covered elements.

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/refinement.eps,scale=0.6}
\end {tabular}
\caption {Example for Greedy Refinement}
\label{refinementexample}
\end{figure}


To overcome the limitation, we propose a greedy refinement algorithm to prune some redundant edges in the gate graph.
The basic idea is to check whether one edge is redundant by searching the shortest paths related to its two endpoints.
Figure \ref{refinementexample} illustrates the idea in checking the redundancy of edge $(u,v)$ highlighted in red.
Here we have shortest paths $(u,v,x_3)$, $(u,v_1,x_3)$, $(u,v,x_4)$, $(u,v_2,x_4)$, $(v,u,x_1)$, $(v,u_1,x_1)$, $(v,u,x_2)$ and $(v,u_2,x_2)$.
In other words, for two endpoints of edge $(u,v)$, if there is a shortest path from one endpoint $u$ to another endpoint $v$'s immediate neighbor $x$,
there is another shortest path from $u$ passing through another vertex to reach $x$.
The dashed lines in the figure demonstrate the alternate shortest paths between one endpoint of the edge and another endpoint's neighbors.
As we know, $x_3$ and $x_4$ are $u$'s 2-hop neighbors, and $x_1$ and $x_2$ are $v$'s 2-hop neighbors.
For $u$ and $v$, since we have more than one shortest paths with 2 edges to reach their 2-hop neighbors,
the removal of edge $(u,v)$ does not affect the goal of reaching all 2-hop neighbors through shortest paths.
Formally, we have the following lemma to allow greedy pruning:

\blemma
\label{prunelemma}
Let $G^\prime=(V^\ast,E^\prime,W)$ be gate graph.
There is an edge $e$ in the gate graph with two endpoints $u$ and $v$, and $H_u(v)=\{x_v\}$ denotes $v$'s immediate neighbors where $(u,v,x_v)$ is shortest path.
Similarly, we define $H_v(u)$ in terms of vertex $v$.
We say edge $e$ is redundant if following conditions are satisfied:

\noindent 1) there is an alternate shortest path $(u,x,x_v)$ between $u$ and $x_v$ for any $x_v \in H_u(v)$ and $x \neq v$;

\noindent 2) there is an alternate shortest path $(v,x,x_u)$ between $v$ and $x_u$ for any $x_u \in H_v(u)$ and $x \neq u$.
\elemma

\input{Figures/GreedyPruning.tex}

Lemma \ref{prunelemma} allows us to evaluate the redundancy of one edge by finding shortest paths with 2 edges related to edge's two endpoints.
Recall that the distance restoration property is guaranteed in the gate graph.
That is, the distance between every 2-hop pairs $(u,v)$ can be computed by combining the distance from $u$ to one of their common neighbors $x$,
and the distance from $x$ to $v$, because distance between $u$ and $v$ is no greater than $2\epsilon$.
The sketch of greedy refinement procedure is described in Algorithm \ref{alg:greedyprune}.

}






\comment{
%% for directed version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% put it into appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given the {\em gates}, we have guaranteed to restore the shortest distance of any pair of vertices by concatenating the local distance and gate distance.
As the {\em gates} are also the vertices in the original graph, the shortest distance between any two {\em gates} is equal to the one from original graph,
thus the first condition of graph simplification problem is satisfied.
In order to investigate the {\em Edge Discovery Problem}, we introduce the {\em Gate Graph} as follows:

\bdefin{\bf (Gate Graph)}
\label{gategraph}
Let $G=(V,E)$ be graph, its discovered gates $V^\ast$ and parameter $\epsilon$.
The weighted graph $G^\prime=(V^\ast, E^\prime,W)$ is gate graph if and only if there is a edge between a pair of gates $u$ and $v$ where $d_G(u,v) \le \epsilon$, and $w(u,v)=d_G(u,v)$.
\edefin

Since the number of gates tends to be significantly smaller than the number vertices in the original graph, the gate graph can be considered as simplified graph in terms of vertices.
According to lemma \ref{restorelemma}, the gate graph satisfies both properties stated in the graph simplification problem, however, the number of edges might not be optimal.
On the other hand, the {\em Edge Discovery Problem} aims to find minimal number of edges connecting {\em gates} while preserving the properties.
Interestingly, we observe that the resulting edges of {\em Edge Discovery Problem} should be the subset of the edge set of gate graph.

\blemma
\label{edgelemma}
Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
The Edge Discover Problem on graph $G$ is equivalent to the problem of extracting minimal number of edges $E^\ast \in E^\prime$ which holds the following property:
\beqnarr
 d_G(u,v)=  \nonumber \\
 min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon} ( d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v) )  \nonumber
\eeqnarr
\elemma

\bproof
Let us first assume that the result of Edge Discovery Problem is edge set $E^\ast$.
In order to hold the property of distance restoration utilizing discovered gates,
for each vertex $u$ in the gate graph $G^\prime$, we require shortest paths which are formed by edges from $E^\ast$ from $u$ to its corresponding gates.
Given this, we first prove that the shortest path from vertex $u$ to one of its corresponding gates actually is a single edge.
That is, there is no gate lying in the shortest path from vertex $u$ to one of its gates.
If there is one gate $x$ lying in the shortest path from $u$ to another gate $v$, we do not need to select $v$ as gate any more.
This is because shortest distances from vertex $u$ to its $(\epsilon+1)-neighbors$ covered by $v$ can also be covered by vertex $x$, as $d_G(u,v)=d_G(u,x)+d_G(x,v)$.
On the other hand, for each vertex, knowing their gates is sufficient to compute all pair of shortest distances as claimed in Lemma \ref{restorelemma}.
This means any edge connecting two vertices with distance greater than $\epsilon$ is redundant.
Thus, the result of Edge Discovery Problem $E^\ast$ is the subset of edges of gate graph $G^\prime$.
Given this, The Edge Discover Problem on graph $G$ can be transformed to the problem of extracting minimal number of edges $E^\ast \in E^\prime$ which holds the property of distance restoration.
\eproof


Based on lemma \ref{restorelemma} and lemma \ref{edgelemma}, for each vertex $u$, only a subset of its incident edges indicating subpaths of shortest paths to their $(\epsilon+1)-neighbors$ are needed.
For each vertex, selecting a subset of edges in gate graph is equivalent to selecting a subset of immediate neighbors (i.e., from $1-neighbors$).
As such, the {\em Edge Discovery Problem} can be converted to many subproblems which is the instance of set cover problem in terms of each vertex.
As stated in lemma \ref{restorelemma}, if each vertex can assess its {\em gates} which lies in the shortest paths from this vertex to its $(\epsilon+1)-neighbors$, then the distance restoration property holds.
In the gate graph, this is much simple since we have guarantee that the distance between any two connected vertices is no greater than $\epsilon$, and the distance from one vertex to its 2-hop neighbors is greater than $\epsilon$.
This motivates an efficient solution based on set cover problem for {\em Edge Discovery Problem}.

Given this, we consider the subproblem of finding a subset of immediate neighbors for vertex $u$.
Let $S=\{v_i\}$ be ground set to be covered, where $v_i$ is 2-hop neighbors from vertex $u$ in the gate graph (i.e., assuming gate graph is unweighted, $v_i$ belongs to $u$'s $2-neighbors$).
For each $u$'s immediate neighbors $x$, it is associated with a subset of vertices $S_u \subseteq S$, where each vertex $v \in S_u$ holds the property $d_G(u,v)=d_G(u,x)+d_G(x,v)$.
In addition, we assign each neighbor $x$ with unit cost, i.e., $cost(x)=1$.
Given this, our goal is to find a subset of neighbors $N^\prime \in Nei(u)$ to the ground set, i.e., $S=\cup_{v \in N^\prime} S_v$, with the minimal cost $\sum_{v \in N^\prime} cost(v)$,
where $Nei(u)$ denotes the immediate neighbors of vertex $u$ in the gate graph.
Also, we can gain the logarithmic approximation result for this subproblem.
For each vertex, its 2-hop neighbors are quite small compared to the number of vertices in the graph, thus the greedy algorithm could be very efficient.
Given this subset of neighbors $N^\prime$, we generate the edges between $u$ and $v \in N^\prime$.
In this procedure, we do not add any new vertex to gate graph, therefore the optimality of the number of vertices is still satisfied.
Putting all those edges together, we have the resulting simplified graph with minimal number vertices and minimal number of edges.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/edgediscovery.eps,scale=0.6}
\end {tabular}
\caption {Illustrative Example for Algorithm \ref{alg:edgediscovery}}
\label{edgediscoverexample}
\end{figure}


\input{Figures/EdgeDiscovery.tex}

The procedure for edge discovery is described in Algorithm \ref{alg:edgediscovery}.
It begins with initializing the resulting edge set $E^\ast$ to be empty set (Line 1).
For each vertex, $u$, we adopt the procedure {\em EdgeSelection} to obtain the minimal number of edges incident to $u$ (Line 3).
Especially, in the procedure {\em EdgeSelection}, for vertex $u$, we use $N^\ast$ to represent the selected edge from $u$ to $x$ belonging to $N^\ast$,
$R$ is the set of covered vertices and $N$ is 2-hop neighbor to be covered (i.e., the ground set).
We first apply breath-first-search traversal to obtain all 2-hop neighbors $N$, and assign $u$'s each immediate neighbor with a subset $N_x$.
Given this, in each iteration, we always choose the vertex $x$ with minimum value of $\frac{1}{N_x \cap (N \setminus R)}$ (Line 6).
Also, $N^\ast$ and $R$ are updated accordingly (Line 7 to Line 8).
The step is proceeded repeatedly until ground set $N$ is totally covered.
Finally, we append edges based on $N^\ast$ to the edge set of simplified graph (Line 10 to Line 12).
Combining the discovered gates $V^\ast$ and the edge set $E^\ast$, the simplified graph $G^\ast$ is returned (Line 5).

\noindent{\bf Running Example:} To gain a better understanding of the set cover procedure, we consider the example illustrated in Figure \ref{edgediscoverexample}.
The figure shows $u$'s immediate neighbors and 2-hop neighbors.
According to set cover framework, each $x_i$ is associated with a set $N_{x_i}$, such that $w(u,v) = w(u,x_i)+(x_i,v)$ and $v \in N_{x_i}$ in the gate graph.
For instance, $x_1$ is associated with the vertex set $\{v_1,v_2,v_3,v_4\}$ and $x_2$ is associated with vertex set $\{v_2,v_7\}$.
Our goal is to find a subset of vertices from $\{x_1,x_2,x_3,x_4\}$ to cover all 2-hop neighbors $\{v_1,v_2,...,v_8\}$.
It is not hard to see that only $x_1$ and $x_4$ are sufficient to all 2-hop neighbors, which are highlighted in red circle.
That it, for vertex $u$, only edges $(u,x_1)$ and $(u,x_4)$ are required in the final simplified graph.

\noindent{\bf Complexity:}
Algorithm \ref{alg:edgediscovery} calls procedure {\em EdgeSelection} $|V|$ times.
For procedure {\em EdgeSelection}, we apply the similar queue technique in Algorithm \ref{alg:gatesdiscovery} to speed up the greedy set cover approach.
In each step, assuming we need to visit $k$ vertices in the queue and $u$'s degree is $d_u$, it takes $O(k(\log d_u+1))$ time.
Thus, the procedure {\em EdgeSelection} at most takes $O(k d_u (\log d_u +1))$ time since the size of $N^\ast$ is no greater than $d_u$.
Overall, the time complexity of Algorithm \ref{alg:edgediscovery} is $O(\sum_{u \in V} k d_u \log d_u)$.

Since the procedure {\em EdgeSelection} can be performed separately on each vertex, we are able to achieve very promising speedup if our algorithm is deployed in distributed computing environment.


\bthm
For each vertex $u$, procedure {\em EdgeSelection} in Algorithm \ref{alg:edgediscovery} has $\ln M$ approximation ratio with respect to the optimal solution,
where $M$ is the number of $u$'s 2-hop neighbors.
\ethm

}





\comment{
In this section, we first introduce an interesting observation from simplified graph which can guarantee the
satisfactory of condition (3). Then, we formulate our graph simplification problem to be an instance of set cover
problem based on this observation. Since the global optimal approach based on set cover problem cannot handle large
graphs, an efficient scheme incorporating refinement step is proposed to address this scalability issue. (consider
approximation problem...)

As we mentioned before, to reach the destination $v$ from the starting vertex $u$ in the graph $G$ utilizing its
simplified graph $G^\prime$, we first get on the appropriate {\em gate} (i.e., one vertex in $G^\prime$ within
$\varepsilon(u)$) in the simplified graph, then go to another {\em gate} within $\varepsilon(v)$ and eventually lead to
the destination $v$ through a shortest path. In other words, each vertex in the graph has to understand what are the
appropriate {\em gates} to get on (or off) $G^\prime$. Since each vertex can directly access the information from other
vertices in its $\varepsilon -ball$, we only need to consider the distance greater than $\epsilon$. Interestingly, for
each vertex $u$ in the graph, we observe that if we can identify a subset of vertices from $G^\prime$ as its {\em
gates} which can lead to the vertices $v^\prime$ where their distances $d_G(u,v^\prime)$ is $\epsilon+1$, we can
restore the distance from $u$ to any its reachable vertex $v$ by following expression: \beqnarr d_G(u,v) = min_{x \in
\varepsilon(u) \wedge y \in \varepsilon(v)} (d_G(u,x) + d_{G^\prime}(x,y) + d_G(y,v)) \eeqnarr Formally, we summarize
the above property as follows:

\blemma For each vertex $u$ in the graph, if we can identify a subset of vertices $L(u) \in V^\prime$ (and $L(u) \in
\varepsilon(u)$) where we always can find a vertex $x \in L(u)$ such that $d_G(u,x) + d_G(x,v) = d_G(u,v)$  and
$d_G(u,v) = \epsilon+1$, then, we can restore the shortest distance between any pair of vertices $u$ and $v$ utilizing
$L(u)$ and $L(v)$ as follows:
\[ d_G(u,v) = min_{x \in L(u) \wedge y \in L(v)} (d_G(u,x) + d_{G^\prime}(x,y) + d_G(y,v)) \]
\elemma

\bproof For any shortest path $P=(v_1,...,v_k)$ whose path length $k$ is greater than $\epsilon$, it should include the
shortest path $P_1=(v_1,...,v_{\epsilon})$ and $P_2=(v_{k-\epsilon+1}, ..., v_k)$. Since we have guarantee that one of
vertex $x \in L(v_1)$ should be in the path $P_1$ and one of vertex $y \in L(v_k)$ should be in the path $P_2$, we have
two vertices $x$ and $y$ in the shortest path $P$. That is, $d_G(v_1,x)$ and $d_G(y,v_k)$ are the shortest distances.
On the other hand, condition (2) tells us $d_{G^\prime}(x,y)$ is the shortest distance between $x$ and $y$ in the
original graph. Putting both together, we have the shortest distance as follows:
\[ d_G(v_1,v_k) = d_G(v_1, x) + d_{G^\prime}(x,y) + d_G(y,v_k) \]
\eproof
}


==> EdgeAlg.tex <==
\section{Our Algorithms}
\label{algorihm}

In this section, we first analyze the problem and introduce an interesting property of $\epsilon-neighbors$ which can guarantee the satisfactory of second condition in graph simplification problem.
Afterward, we formulate the {\em Gates Discovery Problem} to be an instance of set cover problem based on this property.
Given those gates, an efficient approach is proposed to generate the minimal number of edges to connect the gates.



\comment{
\subsection{Algorithm for Edge Discovery Problem}
\label{edgealg}

In this subsection, we study the problem: {\em how to find minimal number of edges to connect the discovered gates while maintaining the property of distance restoration?}
Recall that the shortest distance between any two gates can be restored only using other gates that belongs to their $\epsilon-neighbors$.
This is because the gates are a subset of vertices in the original graph and lemma \ref{restorelemma} is also applicable here.
To explicitly visualize the connectivities among gates, we introduce the concept of {\em Gate Graph} and {\em $k$-hop neighbors} as follows:

\bdefin{\bf (Gate Graph)}
\label{gategraph}
Let $G=(V,E)$ be graph, its discovered gates $V^\ast$ and parameter $\epsilon$.
The weighted graph $G^\prime=(V^\ast, E^\prime,W)$ is gate graph if and only if there is a edge between a pair of gates $u$ and $v$ where $d_G(u,v) \le \epsilon$, and $w(u,v)=d_G(u,v)$.
\edefin

\bdefin{\bf ($k$-hop Neighbors)}
\label{hopneighbor}
Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
In the gate graph, we say vertex $v$ is vertex $u$'s $k$-hop neighbor if and only if there is a shortest path between $u$ and $v$ with $k$ edges in $G^\prime$.
\edefin

In the gate graph, sufficient relationships for computing shortest distance, such as $\epsilon-neighbors$, are preserved, thus all shortest distances of any pair of vertices are maintained.
However, we will see that some edges in the gate graph are not necessary which can be removed without affecting the computation of shortest distance.
On the other hand, the {\em Edge Discovery Problem} aims to find minimal number of edges connecting {\em gates} while preserving the properties.
Fortunately, there is interesting connection between the result of {\em Edge Discovery Problem} and gate graph:
the resulting edges belongs to the edge set of gate graph.

\blemma
\label{edgelemma}
Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
The Edge Discovery Problem on graph $G$ is equivalent to the problem of extracting minimal number of edges from gate graph which holds the following property:
\beqnarr
 d_G(u,v)=  \nonumber \\
 min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon} ( d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v) )  \nonumber
\eeqnarr
\elemma
}

\comment{
\bproof
Let us first assume that the result of Edge Discovery Problem is edge set $E^\ast$.
In the proof, we want to show that $E^\ast$ is the subset of edge set $E^\prime$ in the gate graph.
According to lemma \ref{restorelemma}, for any pair of vertices, there exits a set of gates lying in one of its shortest path, where the distance between two neighboring gates are no greater than $\epsilon$.
Otherwise, at least one vertex pair's shortest distance cannot be restored.
In addition, gates are also a subset of vertices in the original graph, thus each gate also has to connect some other gates within its $\epsilon-neighbors$ to cover all shortest distances to $(\epsilon+1)-neighbors$ in the original graph.
According to our problem definition, we easily see that the distance between one gate with its 2-hop neighbors are greater than $\epsilon$ in the gate graph.
That is, each gate need to connect to some immediate neighbors (i.e., 1-hop neighbors) in order to maintain distance restoration property.
This also means, for each gate, some of its immediate neighbors are redundant.
Thus, the result of Edge Discovery Problem $E^\ast$ is the subset of edges of gate graph $G^\prime$.
\eproof
}

%\bproof
%Let us first assume that the result of Edge Discovery Problem is edge set $E^\ast$.
%In the proof, we want to show that $E^\ast$ is the subset of edge set $E^\prime$ in the gate graph.
%To achieve this, to maintain distance restoration property, we first prove that each gate $v \in V^\ast$ should connect to all its 2-hop neighbors via shortest paths going through $v$'s immediate neighbors.
%Then, we further prove that the above mentioned shortest path actually is an single edge.
%
%According to lemma \ref{restorelemma}, for any pair of vertices, there exits a set of gates lying in one of its shortest path, where the distance between two neighboring gates are no greater than $\epsilon$.
%Otherwise, at least one vertex pair's shortest distance cannot be restored.
%In addition, gates are also a subset of vertices in the original graph, thus each gate also has to connect some other gates within its $\epsilon-neighbors$ to cover all shortest distances to $(\epsilon+1)-neighbors$ in the original graph.
%According to the definition of gate discovery problem, we easily see that the distance between one gate with its 2-hop neighbors are greater than $\epsilon$ in the gate graph.
%Furthermore, for each gate $v$ in the gate graph, there is no guarantee to have $(\epsilon+1)-neighbors$.
%However, if each gate has shortest paths to reach all its 2-hop neighbors, then we are able to compute shortest distance for every pair of gates following similar proof in lemma \ref{restorelemma}.
%Therefore, each gate $v \in V^\ast$ should connect to all its 2-hop neighbors via shortest paths going through $v$'s immediate neighbors.
%
%Given this, we say that there is no gate lying in the shortest path from vertex $u$ to one of its immediate neighbors.
%Considering the original graph, if there is one gate $x$ lying in the shortest path from $u$ to one of its immediate neighbors $v$, we do not need to select $v$ as gate any more.
%This is because shortest distances from vertex $u$ to its $(\epsilon+1)-neighbors$ covered by $v$ can also be covered by vertex $x$, as $d_G(u,v)=d_G(u,x)+d_G(x,v)$.
%
%Recall the edge set of gate graph, it satisfies both conditions and can serve as a feasible solution to retain distance restoration property.
%Thus, the solution of Edge Discovery problem is a subset of edge set in the gate graph.
%%On the other hand, for each vertex, knowing their gates is sufficient to compute all pair of shortest distances as claimed in Lemma \ref{restorelemma}.
%%This means any edge connecting two vertices with distance greater than $\epsilon$ is redundant.
%%Given this, The Edge Discover Problem on graph $G$ can be transformed to the problem of extracting minimal number of edges $E^\ast \in E^\prime$ which holds the property of distance restoration.
%\eproof
%
%
%\begin{figure}
%\centering
%\begin{tabular}{c}
%\psfig{figure=Figures/edgediscovery.eps,scale=0.6}
%\end {tabular}
%\caption {Example for Edge Discovery Problem}
%\label{edgediscoverexample}
%\end{figure}
%
%
%According to lemma \ref{edgelemma}, we transform our edge discovery problem to the problem of finding minimal number of edges from gate graph.
%In addition, following the similar idea of lemma \ref{restorelemma}, in order to hold distance restoration property in the gate graph,
%each gate $u$ should connect to some of its immediate neighbors (i.e., 1-hop neighbors) which cover all shortest distances from $u$ to its 2-hop neighbors.
%Here, we use 1-hop neighbors since gate graph is a weighted graph where each edge weight corresponds to the shortest distance between two connected vertices.
%Also, for each vertex $u$, its immediate neighbors are actually its $\epsilon-neighbros$ since $w(u,v) \le \epsilon$ and $v \in \epsilon-neighbor(u)$,
%and the distance to its 2-hop neighbors are greater than $\epsilon+1$.
%Take figure \ref{edgediscoverexample} as example.
%For vertex $u$, its immediate neighbors are $\{x_1,x_2,x_3,x_4\}$ and 2-hop neighbors are $\{v_1,v_2,...,v_8\}$.
%To hold the property of distance restoration, we can select edge set $\{(u,x_1),(u,x_2),(u,x_3)\}$ or $\{(u,x_1),(u,x_3),(u,x_4)\}$ to cover all 2-hop neighbors.
%
%However, we cannot select the edge set for each vertex individually.
%The central challenge here is original graph is undirected graph and each edge serves as the intermediate edge within different shortest paths from both directions.
%More importantly, the effectiveness of the edge relies on its incident edges, meaning one edge should incorporate with other edges to form the shortest path.
%For instance, in order to use edge $(u,x_1)$ as the edge in the shortest path from $u$ to $v_1$, we have to guarantee that the edge $(x_1,v_1)$ is also chosen.
%Therefore, we cannot directly apply traditional set cover approach to find the minimal number of edges from gate graph.
%Interestingly, we find that our problem can be transformed into a new variant of set cover problem, referred to as {\em Set-Cover-with-Pairs} (SCP) problem.
%
%\bdefin{\bf (Set-Cover-with-Pairs Problem ~\cite{HS05})}
%\label{scpdef}
%Let $U$ be the ground set and let $S = \{1, \ldots, M\}$ be a set of objects, where each object $i\in S$ has a non-negative cost $w_i$. For every $\{i,j\}\subseteq S$, let $\mathcal{C}(i, j)$ be the collection of elements in $U$ covered by the pair $\{i, j\}$. The objective of the set cover with pairs (SCP) problem is to find a subset $S^\prime \subseteq S$ such that
% $\mathcal{C}(S^\prime) =\bigcup_{\{i,j\}\subseteq S^\prime} \mathcal{C}(i, j) = U.$
% with a minimum covering cost $\sum_{i\in S} w_i$.
%We refer to the special case in which each object has  a unit weight ($w_i=1$) as the \textbf{cardinality SCP} problem.
% \edefin
%
%Before we go to the solution, we first define {\em edge coverage} here:
%
%\bdefin{\bf (Edge Coverage)}
%Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
%We have two edges $e_1=(u,x) \in E^\prime$, $e_2=(y,v) \in E^\prime$, and vertex pair $(u,v)$ where $u$ and $v$ are each other's 2-hop neighbor.
%We say $e_1$ and $e_2$ cover vertex pair $(u,v)$ if and only $x$ and $y$ are the same vertex and $d_G(u,v)=w(u,x)+w(y,v)$.
%\edefin
%
%That is, edges $e_1=(u,x)$ and $e_2=(y,v)$ constitutes the shortest path from vertex $u$ to $v$ in the gate graph.
%Given this, we have the ground set $U=\{(u_0,v_0),(u_1,v_1),...\}$ where $u_i$ and $v_i$ are each other's 2-hop neighbor.
%Then, we also have the edge set $E^\prime$ as the object set $S$ where each edge is assigned with unit cost.
%Also, each pair of edge $e_1$ and $e_2$ is associated with single vertex pair $\mathcal{C}(e_1,e_2)$ which can be {\em covered} by them (i.e., $e_1$ and $e_2$ are concatenated to be a shortest path between such pair).
%Our goal is to find a subset of edges $E^\ast \in E^\prime$ such that $\mathcal{C}(E^\ast)=\bigcup_{\{e_i,e_j\}\subseteq E^\ast} \mathcal{C}(e_i, e_j) = U$,
%with minimum cost $|E^\ast|$ (i.e., minimum number of edges within $E^\ast$).
%Since our problem is the instance of SCP problem which has been proven to be NP-hard, we have:
%
%\bthm
%The edge discovery problem on gate graph is NP-hard.
%\ethm
%
%
%\begin{figure}
%    \label{expfig}
%    \centering
%    \mbox{
%        \subfigure[Gate Graph] {\epsfig{figure=Figures/gategraphexample.eps,scale=0.6} \label{fig:gategraph}}
%        \subfigure[Set-Cover-with-Pairs Setting]{\epsfig{figure=Figures/setcoverpairs.eps,scale=0.6}\label{fig:setcoverwithpairs}}
%    }
%    \label{scpexample}
%    \caption{Example for Edge Discovery Algorithm}
%\end{figure}
%
%Let us consider the example in Figure~\ref{scpexample}, where gate graph is shown in Figure~\ref{fig:gategraph}.
%Note that, we omit the edge weight in Figure~\ref{fig:gategraph} for simplification, and the shortest paths including 3 vertices are specified in the lower part.
%As discussed, each shortest path identified by two endpoints is make up of two edges which serve as objects in the traditional Set-Cover-with-Pairs problem (Definition \ref{scpdef}).
%And two endpoints forms a vertex pair included in the ground set.
%According to underlying shortest paths, we visualize the edge-pair covering structure in Figure~\ref{fig:setcoverwithpairs}.
%There is an edge in the covering structure if and only if two edges form a shortest path in the gate graph.
%For instance, there is a shortest path $(v_2,v_8,v_7)$ which is the concatenation of edge $(v_2,v_8)$ and edge $(v_7,v_8)$.
%Therefore, we connect $(v_2,v_8)$ and $(v_7,v_8)$ in the edge-pair covering structure.
%Also, shortest path between $v_2$ and $v_7$ can be covered by edge $(v_2,v_3)$ and $(v_3,v_7)$.

\comment{
\input{Figures/EdgeDiscovery.tex}

Borrowing the idea for solving SCP problem in~\cite{DBLP:conf/fsttcs/HassinS05}, we describe our procedure for edge discovery problem in Algorithm \ref{alg:edgediscovery}.
It begins with initializing the resulting edge set $E^\ast$ and intermediate cover set $R$ to be empty set (Line 1 to Line 2).
For each vertex $u$, we adopt procedure {\em BFS} similar to Algorithm \ref{alg:bfssetcover} to obtain the ground set $U$ and each vertex's associated vertex pairs (Line 3 to Line 5).
In the main while loop (Line 6 to Line 15), for each iteration, we greedily select an edge or an pair of edges which can minimize the cost
$\frac{1}{|\mathcal{C}(E^\ast \cup\{e_i\})\backslash\mathcal{C}(E^\ast)|}$ or $\frac{2}{|\mathcal{C}(E^\ast\cup\{e_i,e_j\})\backslash\mathcal{C}(E^\ast)|}$.
Then, we update the resulting set $E^\ast$ and intermediate cover set $R$ correspondingly (Line 9 to Line 14).
We repeat such iteration until entire ground set $U$ is covered.
Combining the discovered gates $V^\ast$ and the edge set $E^\ast$, the simplified graph $G^\ast$ is returned (Line 16).


\subsubsection{Alternate Greedy Algorithm}
\label{approxgreedy}

Aforementioned greedy algorithm has been proved to have an $O(\sqrt{N \log N})$ approximation ratio, where $N = |U|$ is the size of ground set.
Here, we present an alternate greedy algorithm which considers the potential benefit to evaluate each edge in the selection procedure.
Our greedy algorithm works as follows: {\em each time we select an edge according to our defined criterion, until all elements in the ground set, i.e., all 2-hop vertex pairs in the gate graph, have been covered.}

To describe our edge-selection criterion, we introduce the following definitions:
Let $U$ be the ground set and $R$ be the set recording the already covered vertex: $R \subseteq U$.
Let $S$ be the set of already selected edges and let $\overline{S}$ denote the unused edges in $E^\prime$, $\overline{S}=E^\prime \setminus S$.
Using the graph formulation, we construct a graph $\mathcal{G}=(\mathcal{V}, \mathcal{E})$, where each vertex in $\mathcal{V}$ represents one edge in $E^\prime$.
And, there is an edge $(e_x,e_y) \in \mathcal{E}$ if and only $e_x$ and $e_y$ in the gate graph concatenate with each other to form a shortest path from one endpoint of $e_x$ to one endpoint of $e_y$.
In addition, each edge $\mathcal{e} \in \mathcal{E}$ is associated with one vertex pair corresponding to two endpoints of covered shortest path.

Given this, in the graph $\mathcal{G}$, we assume at some iteration, the vertex $v$ is to be selected.
Let $\mathcal{E}(v)$ denotes the set of edges in $\mathcal{G}$ adjacent to $v$.
Then $\mathcal{E}(v)$ covers a set of vertex pairs in $U \setminus R$.
We categorize $\mathcal{E}(v)$ into two parts:
1) one part is immediately covered by selecting $v$;
in other words, $v$ will work directly on those already selected nodes in $S$, denoted as $S_{v}$, to cover this part of the elements;
2) the other part is those elements which may be covered in the future when selecting nodes in $Z_{v}$, where $Z_{v}\subseteq \overline{S}$ and each node in $Z_{v}$ is adjacent to $v$.
It is easy to see $|S_{v}|$ is exactly how many new elements will be covered if we select $v$ at step $i$,
and $|Z_{v}|$ is how many new elements will be {\em potentially} covered as a consequence of selecting $v$.
In other words, $|S_{v}|+|Z_{v}|$ is the upper bound of the number of elements which can be covered by selecting node $v$.
In our algorithm, at each iteration, we select node $v$ from $\overline{S}$ with minimum $\frac{1}{|S_{v}|+|Z_{v}|}$.
Intuitively, we can see that our algorithm with its criteria is ``optimistic'' or ''far-sighted'' as it always selects the node with ``maximal potential'' ($\max {|S_{v}|+|Z_{v}|}$) .
However, the original greedy algorithm~\cite{DBLP:conf/fsttcs/HassinS05} is ``pessimistic''  or ``short-sighted'' as it always selects the node with the immediate best output ($\max {|S_{v}|}= \max {|\mathcal{C}(R\cup\{i\})\backslash\mathcal{C}(R)|}$).
The sketch of new greedy algorithm is outlined in Algorithm~\ref{alg:newedgediscovery}.

\input{Figures/GatesDiscoveryNew.tex}

}

\comment{
\subsection{Greedy Refinement Algorithm}
\label{greedyrefine}

The traditional greedy algorithm for Set-Cover-with-Pairs problem yields $O(\sqrt(N \log N))$ approximation ratio, where $N$ is the number of size of ground set $N = |U|$.
In our problem for edge discovery, the size of ground set is the same with the number of shortest paths containing 2 edges in the gate graph.
In the worst case, $N$ could be very large and the approximation ratio is not attractive enough.
Moreover, as speedup technique with queue for greedy algorithm of set cover problem is not applicable here,
it is very time consuming to choose ``best'' object in each iteration by scanning all remaining objects and checking their covered elements.

\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/refinement.eps,scale=0.6}
\end {tabular}
\caption {Example for Greedy Refinement}
\label{refinementexample}
\end{figure}


To overcome the limitation, we propose a greedy refinement algorithm to prune some redundant edges in the gate graph.
The basic idea is to check whether one edge is redundant by searching the shortest paths related to its two endpoints.
Figure \ref{refinementexample} illustrates the idea in checking the redundancy of edge $(u,v)$ highlighted in red.
Here we have shortest paths $(u,v,x_3)$, $(u,v_1,x_3)$, $(u,v,x_4)$, $(u,v_2,x_4)$, $(v,u,x_1)$, $(v,u_1,x_1)$, $(v,u,x_2)$ and $(v,u_2,x_2)$.
In other words, for two endpoints of edge $(u,v)$, if there is a shortest path from one endpoint $u$ to another endpoint $v$'s immediate neighbor $x$,
there is another shortest path from $u$ passing through another vertex to reach $x$.
The dashed lines in the figure demonstrate the alternate shortest paths between one endpoint of the edge and another endpoint's neighbors.
As we know, $x_3$ and $x_4$ are $u$'s 2-hop neighbors, and $x_1$ and $x_2$ are $v$'s 2-hop neighbors.
For $u$ and $v$, since we have more than one shortest paths with 2 edges to reach their 2-hop neighbors,
the removal of edge $(u,v)$ does not affect the goal of reaching all 2-hop neighbors through shortest paths.
Formally, we have the following lemma to allow greedy pruning:

\blemma
\label{prunelemma}
Let $G^\prime=(V^\ast,E^\prime,W)$ be gate graph.
There is an edge $e$ in the gate graph with two endpoints $u$ and $v$, and $H_u(v)=\{x_v\}$ denotes $v$'s immediate neighbors where $(u,v,x_v)$ is shortest path.
Similarly, we define $H_v(u)$ in terms of vertex $v$.
We say edge $e$ is redundant if following conditions are satisfied:

\noindent 1) there is an alternate shortest path $(u,x,x_v)$ between $u$ and $x_v$ for any $x_v \in H_u(v)$ and $x \neq v$;

\noindent 2) there is an alternate shortest path $(v,x,x_u)$ between $v$ and $x_u$ for any $x_u \in H_v(u)$ and $x \neq u$.
\elemma

\input{Figures/GreedyPruning.tex}

Lemma \ref{prunelemma} allows us to evaluate the redundancy of one edge by finding shortest paths with 2 edges related to edge's two endpoints.
Recall that the distance restoration property is guaranteed in the gate graph.
That is, the distance between every 2-hop pairs $(u,v)$ can be computed by combining the distance from $u$ to one of their common neighbors $x$,
and the distance from $x$ to $v$, because distance between $u$ and $v$ is no greater than $2\epsilon$.
The sketch of greedy refinement procedure is described in Algorithm \ref{alg:greedyprune}.

}






\comment{
%% for directed version
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% put it into appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Given the {\em gates}, we have guaranteed to restore the shortest distance of any pair of vertices by concatenating the local distance and gate distance.
As the {\em gates} are also the vertices in the original graph, the shortest distance between any two {\em gates} is equal to the one from original graph,
thus the first condition of graph simplification problem is satisfied.
In order to investigate the {\em Edge Discovery Problem}, we introduce the {\em Gate Graph} as follows:

\bdefin{\bf (Gate Graph)}
\label{gategraph}
Let $G=(V,E)$ be graph, its discovered gates $V^\ast$ and parameter $\epsilon$.
The weighted graph $G^\prime=(V^\ast, E^\prime,W)$ is gate graph if and only if there is a edge between a pair of gates $u$ and $v$ where $d_G(u,v) \le \epsilon$, and $w(u,v)=d_G(u,v)$.
\edefin

Since the number of gates tends to be significantly smaller than the number vertices in the original graph, the gate graph can be considered as simplified graph in terms of vertices.
According to lemma \ref{restorelemma}, the gate graph satisfies both properties stated in the graph simplification problem, however, the number of edges might not be optimal.
On the other hand, the {\em Edge Discovery Problem} aims to find minimal number of edges connecting {\em gates} while preserving the properties.
Interestingly, we observe that the resulting edges of {\em Edge Discovery Problem} should be the subset of the edge set of gate graph.

\blemma
\label{edgelemma}
Let $G=(V,E)$ be original graph and $G^\prime=(V^\ast,E^\prime,W)$ be its corresponding gate graph.
The Edge Discover Problem on graph $G$ is equivalent to the problem of extracting minimal number of edges $E^\ast \in E^\prime$ which holds the following property:
\beqnarr
 d_G(u,v)=  \nonumber \\
 min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon} ( d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v) )  \nonumber
\eeqnarr
\elemma

\bproof
Let us first assume that the result of Edge Discovery Problem is edge set $E^\ast$.
In order to hold the property of distance restoration utilizing discovered gates,
for each vertex $u$ in the gate graph $G^\prime$, we require shortest paths which are formed by edges from $E^\ast$ from $u$ to its corresponding gates.
Given this, we first prove that the shortest path from vertex $u$ to one of its corresponding gates actually is a single edge.
That is, there is no gate lying in the shortest path from vertex $u$ to one of its gates.
If there is one gate $x$ lying in the shortest path from $u$ to another gate $v$, we do not need to select $v$ as gate any more.
This is because shortest distances from vertex $u$ to its $(\epsilon+1)-neighbors$ covered by $v$ can also be covered by vertex $x$, as $d_G(u,v)=d_G(u,x)+d_G(x,v)$.
On the other hand, for each vertex, knowing their gates is sufficient to compute all pair of shortest distances as claimed in Lemma \ref{restorelemma}.
This means any edge connecting two vertices with distance greater than $\epsilon$ is redundant.
Thus, the result of Edge Discovery Problem $E^\ast$ is the subset of edges of gate graph $G^\prime$.
Given this, The Edge Discover Problem on graph $G$ can be transformed to the problem of extracting minimal number of edges $E^\ast \in E^\prime$ which holds the property of distance restoration.
\eproof


Based on lemma \ref{restorelemma} and lemma \ref{edgelemma}, for each vertex $u$, only a subset of its incident edges indicating subpaths of shortest paths to their $(\epsilon+1)-neighbors$ are needed.
For each vertex, selecting a subset of edges in gate graph is equivalent to selecting a subset of immediate neighbors (i.e., from $1-neighbors$).
As such, the {\em Edge Discovery Problem} can be converted to many subproblems which is the instance of set cover problem in terms of each vertex.
As stated in lemma \ref{restorelemma}, if each vertex can assess its {\em gates} which lies in the shortest paths from this vertex to its $(\epsilon+1)-neighbors$, then the distance restoration property holds.
In the gate graph, this is much simple since we have guarantee that the distance between any two connected vertices is no greater than $\epsilon$, and the distance from one vertex to its 2-hop neighbors is greater than $\epsilon$.
This motivates an efficient solution based on set cover problem for {\em Edge Discovery Problem}.

Given this, we consider the subproblem of finding a subset of immediate neighbors for vertex $u$.
Let $S=\{v_i\}$ be ground set to be covered, where $v_i$ is 2-hop neighbors from vertex $u$ in the gate graph (i.e., assuming gate graph is unweighted, $v_i$ belongs to $u$'s $2-neighbors$).
For each $u$'s immediate neighbors $x$, it is associated with a subset of vertices $S_u \subseteq S$, where each vertex $v \in S_u$ holds the property $d_G(u,v)=d_G(u,x)+d_G(x,v)$.
In addition, we assign each neighbor $x$ with unit cost, i.e., $cost(x)=1$.
Given this, our goal is to find a subset of neighbors $N^\prime \in Nei(u)$ to the ground set, i.e., $S=\cup_{v \in N^\prime} S_v$, with the minimal cost $\sum_{v \in N^\prime} cost(v)$,
where $Nei(u)$ denotes the immediate neighbors of vertex $u$ in the gate graph.
Also, we can gain the logarithmic approximation result for this subproblem.
For each vertex, its 2-hop neighbors are quite small compared to the number of vertices in the graph, thus the greedy algorithm could be very efficient.
Given this subset of neighbors $N^\prime$, we generate the edges between $u$ and $v \in N^\prime$.
In this procedure, we do not add any new vertex to gate graph, therefore the optimality of the number of vertices is still satisfied.
Putting all those edges together, we have the resulting simplified graph with minimal number vertices and minimal number of edges.


\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/edgediscovery.eps,scale=0.6}
\end {tabular}
\caption {Illustrative Example for Algorithm \ref{alg:edgediscovery}}
\label{edgediscoverexample}
\end{figure}


\input{Figures/EdgeDiscovery.tex}

The procedure for edge discovery is described in Algorithm \ref{alg:edgediscovery}.
It begins with initializing the resulting edge set $E^\ast$ to be empty set (Line 1).
For each vertex, $u$, we adopt the procedure {\em EdgeSelection} to obtain the minimal number of edges incident to $u$ (Line 3).
Especially, in the procedure {\em EdgeSelection}, for vertex $u$, we use $N^\ast$ to represent the selected edge from $u$ to $x$ belonging to $N^\ast$,
$R$ is the set of covered vertices and $N$ is 2-hop neighbor to be covered (i.e., the ground set).
We first apply breath-first-search traversal to obtain all 2-hop neighbors $N$, and assign $u$'s each immediate neighbor with a subset $N_x$.
Given this, in each iteration, we always choose the vertex $x$ with minimum value of $\frac{1}{N_x \cap (N \setminus R)}$ (Line 6).
Also, $N^\ast$ and $R$ are updated accordingly (Line 7 to Line 8).
The step is proceeded repeatedly until ground set $N$ is totally covered.
Finally, we append edges based on $N^\ast$ to the edge set of simplified graph (Line 10 to Line 12).
Combining the discovered gates $V^\ast$ and the edge set $E^\ast$, the simplified graph $G^\ast$ is returned (Line 5).

\noindent{\bf Running Example:} To gain a better understanding of the set cover procedure, we consider the example illustrated in Figure \ref{edgediscoverexample}.
The figure shows $u$'s immediate neighbors and 2-hop neighbors.
According to set cover framework, each $x_i$ is associated with a set $N_{x_i}$, such that $w(u,v) = w(u,x_i)+(x_i,v)$ and $v \in N_{x_i}$ in the gate graph.
For instance, $x_1$ is associated with the vertex set $\{v_1,v_2,v_3,v_4\}$ and $x_2$ is associated with vertex set $\{v_2,v_7\}$.
Our goal is to find a subset of vertices from $\{x_1,x_2,x_3,x_4\}$ to cover all 2-hop neighbors $\{v_1,v_2,...,v_8\}$.
It is not hard to see that only $x_1$ and $x_4$ are sufficient to all 2-hop neighbors, which are highlighted in red circle.
That it, for vertex $u$, only edges $(u,x_1)$ and $(u,x_4)$ are required in the final simplified graph.

\noindent{\bf Complexity:}
Algorithm \ref{alg:edgediscovery} calls procedure {\em EdgeSelection} $|V|$ times.
For procedure {\em EdgeSelection}, we apply the similar queue technique in Algorithm \ref{alg:gatesdiscovery} to speed up the greedy set cover approach.
In each step, assuming we need to visit $k$ vertices in the queue and $u$'s degree is $d_u$, it takes $O(k(\log d_u+1))$ time.
Thus, the procedure {\em EdgeSelection} at most takes $O(k d_u (\log d_u +1))$ time since the size of $N^\ast$ is no greater than $d_u$.
Overall, the time complexity of Algorithm \ref{alg:edgediscovery} is $O(\sum_{u \in V} k d_u \log d_u)$.

Since the procedure {\em EdgeSelection} can be performed separately on each vertex, we are able to achieve very promising speedup if our algorithm is deployed in distributed computing environment.


\bthm
For each vertex $u$, procedure {\em EdgeSelection} in Algorithm \ref{alg:edgediscovery} has $\ln M$ approximation ratio with respect to the optimal solution,
where $M$ is the number of $u$'s 2-hop neighbors.
\ethm

}





\comment{
In this section, we first introduce an interesting observation from simplified graph which can guarantee the
satisfactory of condition (3). Then, we formulate our graph simplification problem to be an instance of set cover
problem based on this observation. Since the global optimal approach based on set cover problem cannot handle large
graphs, an efficient scheme incorporating refinement step is proposed to address this scalability issue. (consider
approximation problem...)

As we mentioned before, to reach the destination $v$ from the starting vertex $u$ in the graph $G$ utilizing its
simplified graph $G^\prime$, we first get on the appropriate {\em gate} (i.e., one vertex in $G^\prime$ within
$\varepsilon(u)$) in the simplified graph, then go to another {\em gate} within $\varepsilon(v)$ and eventually lead to
the destination $v$ through a shortest path. In other words, each vertex in the graph has to understand what are the
appropriate {\em gates} to get on (or off) $G^\prime$. Since each vertex can directly access the information from other
vertices in its $\varepsilon -ball$, we only need to consider the distance greater than $\epsilon$. Interestingly, for
each vertex $u$ in the graph, we observe that if we can identify a subset of vertices from $G^\prime$ as its {\em
gates} which can lead to the vertices $v^\prime$ where their distances $d_G(u,v^\prime)$ is $\epsilon+1$, we can
restore the distance from $u$ to any its reachable vertex $v$ by following expression: \beqnarr d_G(u,v) = min_{x \in
\varepsilon(u) \wedge y \in \varepsilon(v)} (d_G(u,x) + d_{G^\prime}(x,y) + d_G(y,v)) \eeqnarr Formally, we summarize
the above property as follows:

\blemma For each vertex $u$ in the graph, if we can identify a subset of vertices $L(u) \in V^\prime$ (and $L(u) \in
\varepsilon(u)$) where we always can find a vertex $x \in L(u)$ such that $d_G(u,x) + d_G(x,v) = d_G(u,v)$  and
$d_G(u,v) = \epsilon+1$, then, we can restore the shortest distance between any pair of vertices $u$ and $v$ utilizing
$L(u)$ and $L(v)$ as follows:
\[ d_G(u,v) = min_{x \in L(u) \wedge y \in L(v)} (d_G(u,x) + d_{G^\prime}(x,y) + d_G(y,v)) \]
\elemma

\bproof For any shortest path $P=(v_1,...,v_k)$ whose path length $k$ is greater than $\epsilon$, it should include the
shortest path $P_1=(v_1,...,v_{\epsilon})$ and $P_2=(v_{k-\epsilon+1}, ..., v_k)$. Since we have guarantee that one of
vertex $x \in L(v_1)$ should be in the path $P_1$ and one of vertex $y \in L(v_k)$ should be in the path $P_2$, we have
two vertices $x$ and $y$ in the shortest path $P$. That is, $d_G(v_1,x)$ and $d_G(y,v_k)$ are the shortest distances.
On the other hand, condition (2) tells us $d_{G^\prime}(x,y)$ is the shortest distance between $x$ and $y$ in the
original graph. Putting both together, we have the shortest distance as follows:
\[ d_G(v_1,v_k) = d_G(v_1, x) + d_{G^\prime}(x,y) + d_G(y,v_k) \]
\eproof
}


==> KSkipCover.tex <==
\section{Discussion on k-skip cover}
\label{ksipcover}

In this section, we will discuss $k$-skip cover which is highly related to gate-vertex set.
In particular, we first explore the relationship between them.
Then, we extend our theoretical results and algorithmic solution to tackle {\em minimum $k$-skip cover problem} which is still open.
Also, we prove the NP-hardness of {\em minimum $k$-skip cover problem}.


\comment{
\begin{figure}
\centering
\begin{tabular}{c}
\psfig{figure=Figures/skipcoverexamp.eps,scale=0.6}
\end {tabular}
\caption {Example for difference between $k$-skip cover and gate-vertex set}
\label{skipcoverexamp}
\end{figure}
}

\subsection{Relationship between gate-vertex set and $k$-skip cover}

The notion of $k$-skip cover~\cite{Tao11} is a subset of ``essential'' vertices capturing the information of shortest paths in the
original graph.
Specially, shortest path between any vertex pair can be compactly represented by a sequence of vertices from $k$-skip cover,
such that every two neighboring vertices are at most $k$ steps far apart from each other.
We first repeat the concept of $k$-skip cover to facilitate the discussion:

\bdefin {\bf ($k$-skip cover)}
Given graph $G=(V,E)$, a subset $V^\ast \subseteq V$ is $k$-skip cover which holds the following property:
for any vertex pair $(s,t) \in V \times V$ with distance $k-1$, there exists one shortest path $p_{s,t}$ between them,
where $V^\ast$ contains at least one vertex in $p_{s,t}$.
\edefin

From the perspective of shortest path representation, $k$-skip cover is rather similar to gate-vertex set. That is, the
shortest path between any vertex pair in gate-vertex set can be restored by concatenating several gate vertices such
that distance between every two neighboring gate vertices are at most $\epsilon$. As discussed in
Section~\ref{gatediscovery}, we have demonstrate their relationship by lemma~\ref{kscgv}. Here, we further explore them and
observe an interesting relationship. Let $G_\epsilon$, $S_k$ denote gate-vertex set with parameter $\epsilon$ and
$k$-skip cover, respectively. And their sizes are expressed as $|G_\epsilon|$ and $|S_k|$ correspondingly.


\bthm
The relationship between gate-vertex set and $k$-skip cover are:
\[ G_1 \subseteq S_2 \subseteq G_3 \subseteq ... G_{i-1} \subseteq S_i \subseteq G_{i+1} \subseteq ... \]
In other words, we can say $min |G_{i-1}| \ge min |S_i| \ge min |G_{i+1}|$,
where $min|G_\epsilon|$ and $min|S_k|$ are minimum cardinality of gate-vertex set with parameter $\epsilon$ and $k$-skip cover, respectively.
\ethm


To obtain the above result, we first provide the following lemma:

\blemma
\label{gvksc}
Given graph $G=(V,E)$,
if parameters $\epsilon$ of gate-vertex set and $k$ of $k$-skip cover satisfy condition $k = \epsilon+1$,
gate-vertex set $V^\ast$ is a $k$-skip cover.
\elemma
\bproof
We prove it by contradiction.
Assuming $V^\ast$ is not a $k$-skip cover, there should exist one vertex pair $(u,v)$ with distance $k-1$
such that $V^\ast$ does not contain any vertex from any shortest path $p_{u,v}$ between them.
This means, we do not have a vertex $x\in V^\ast$ for vertex pair $(u,v)$ with distance $\epsilon$ (since $\epsilon=k-1$),
such that $d(u,x)+d(x,v)=d(u,v)$.
Therefore, $V^\ast$ cannot cover vertex pair $\epsilon$ which contradicts with the definition of gate-vertex set.
\eproof


Combining lemma~\ref{kscgv} and lemma~\ref{gvksc}, the relationship of $G_{i-1} \subseteq S_i \subseteq G_{i+1}$ is easily observed.
Since gate-vertex set $G_{i-1}$ is a subset of $i$-skip cover $S_i$, the smallest number of $S_i$ is guaranteed to be no greater than that of $G_{i-1}$.
Hence, we have $min |G_{i-1}| \ge min |S_i|$. Similar inequality holds for $S_i$ and $G_{i+1}$.
In this sense, any application or scheme utilizing $k$-skip cover, such as shortest path query and graph visualization,
can adopt gate-vertex set to achieve the same goal, and vice versa.
Inspiring by this spirit, we extent our algorithmic solution for minimum gate-vertex set to minimum $k$-skip which is still unexplored in the following subsection.



\comment{
% to be rewritten
However, the lemma is not true conversely, i.e., $k$-skip cover is not necessarily a gate-vertex when $k=\epsilon+1$.
To gain better understanding of difference between both concepts, we consider the most simple scenario, shortest path of length $\epsilon$ and $\epsilon+2=k$.
As shown in Figure~\ref{skipcoverexamp}, the upper one highlights $4$-skip cover and the lower one indicates a gate-vertex set with $\epsilon=2$.
We can see, in $4$-skip cover, staring point $s$ is qualified to be one representative of first $4$ consecutive vertices.
However, in gate-vertex set with $\epsilon=2$, we seek a subset of vertices to cover the vertex pairs with distance $\epsilon+1$ (i.e., $3$).
For the shortest path between $s$ and $t$, only the vertices without two endpoints are considered as candidates of gate vertices,
since two endpoints cannot serve as intermediates to restore the shortest distance.
Generally speaking, the notion of gate-vertex set is even stronger than that of $k$-skip cover.
Also, any application utilizing $k$-skip cover, such as shortest path query and graph visualization, can adopt gate-vertex set to achieve the same goal.
}

\subsection{Minimum $k$-skip cover}
\label{minkskipcover}

As mentioned in \cite{Tao11}, how to design a deterministic algorithm of minimum $k$-skip cover problem is a open problem so far.
To be self-contained, we clarify the problem definition as follows.

\bdefin {\bf (Minimum $k$-skip cover problem)}
Given graph $G=(V,E)$, we try to discover a $k$-skip cover with minimum cardinality.
\edefin


%\noindent{\bf Problem Complexity: }
%We prove the NP-hardness of minimum $k$-skip cover problem by reducing vertex cover problem.

\bthm %{\bf (NP-hardness of Minimal $k$-Skip Cover Problem)}
\label{nphardskipcover}
Minimum $k$-skip cover problem is NP-hard.
\ethm

\bproof
Basic idea is to reduce the instance of Vertex-Cover problem to the instance of $k$-Skip Cover problem with $k=2$.
In the following, we consider the decision version of both problems.
Given undirected graph $G=(V,E)$ and an integer $m$, the decision problem of vertex cover is to check whether there is a subset of vertices $V^\prime \subseteq V$ with size at most $m$
so that for every edge $(u,v) \in E$ either $u \in V^\prime$ or $v \in V^\prime$.
Similarly, the decision version of $k$-skip cover problem decides if there is a subset of vertices $V^\prime$ with size at most $m$ covers all shortest paths with length $k-1$ in the graph.
Next we show the transformation from an instance of Vertex-Cover to an instance of $k$-Skip Cover:

\noindent 1) Let us assume $V^\prime$ is a solution for $k$-Skip Cover problem with $k=2$.
It is not hard to observe that shortest paths with $k=2$ vertices are actually edges in $G$, and at least one endpoint of such shortest path is included in $V^\ast$.
Since all such shortest paths are covered, so are whole edges in $G$, therefore, $V^\ast$ is a solution to Vertex-Cover problem.

\noindent 2) On the other hand, assuming $V^\ast$ is a solution for Vertex-Cover problem, let us consider a pair of vertices $(s,t) \in V \times V$ and any shortest path $P_{st}$ between them.
Clearly, there exists some vertices from $V^\ast$ being the endpoint of any shortest path $P_{st}$, and thus $V^\ast$ is also a solution to $k$-Skip Cover regarding $k=2$.
\eproof


\noindent{\bf Size of Minimum $k$-Skip Cover: }

Along the line discussed in subsection \ref{sizegateset}, all theoretical results holds for minimum $k$-skip cover.
Specially, for any graph $G=(V,E)$ with $|V|=n$, a $\frac{k}{n}-net$ $V^\ast$ of $(V,P)$ is a $k$-skip cover of $G$, where $P$ is USPS and contains one shortest path for each vertex pair.
Using $\epsilon$-net theorem, we have following results:

\bthm
Given graph $G=(V,E)$ with $|V|=n$, there exists a $k$-skip cover of size $O(\frac{n}{k} \log \frac{n}{k})$.
\ethm

\bthm
Given graph $G=(V,E)$ with $|V|=n$, the size of minimum $k$-skip cover is bounded by $O(\frac{n}{k} \log \frac{n}{k})$.
\ethm


\noindent{\bf Set-Cover Based Solution: }

We transform minimum $k$-skip cover problem to an instance of set cover.
Let $U=\{(u,v) | d(u,v) = k-1\}$ be the ground set, containing all vertex pairs with distance $k-1$.
For each vertex $x$ in the graph, it is associated with a set of vertex pairs $C_x=\{(u,v) | d(u,v)=d(u,x)+d(x,y) =k\}$,
containing all vertex pairs with distance $k$ and there is shortest path between them going through it.
It is worthwhile to note that, shortest path $p_{u,v}$ also goes through its two endpoints $u$ and $v$,
i.e., $u \in C_u$ and $v \in C_v$ which are not true in minimum gate-vertex set problem.
The minimal $k$-skip cover is a subset of vertices $V^\ast \in V$ which covers the ground set,
i.e., $U = \bigcup_{v \in V^\ast} C_v$, with minimal cardinality $|V^\ast|$.
In this sense, we can apply aforementioned algorithm for minimum gate-vertex set to solve it.


==> Prob.tex <==
\section{Theoretical Basis}
\label{probdef}

Based on the definition of the gate-vertex set,  to simply determine whether a set of vertices $V_s$ is a set of  gate vertices, 
the straightforward approach needs to explicitly verify the distance of each {\bf non-local pair}  $(u,v)$ can be recovered through a sequence of consecutive local pairs, there is a vertex sequence (formed by consecutive {\bf local pairs}) from $u$ to $v$, ($u,v_1$), ($v_1,v_2$), $\cdots$, ($v_k,v$), where each intermediate vertices $v_1, v_2, \cdots, v_k$ belong $V_s$. 
Clearly, this can be rather expensive and cannot help us to discover the minimal set of gate vertices. 
In this section, we first introduce an alternative (and much simplified) condition which can help us determine whether a set of vertices are gate vertices. 
Based on this condition, we  will  then prove the NP-hardness of the gate-vertex discovering problem. 

\bthm{\bf (Equivalent Condition)} 
\label{equivalent}
Given an undirected graph $G=(V,E)$ and the parameter $\epsilon$, if a subset of vertices $V^\prime \subseteq V$ satisfy the following condition: for any {\bf non-local pair} $u$ and $v$, there is $x,y \in V^\prime$, 
\beqnarr
 d(u,v)= d(u,x) + d(x,y) + d(y,v), mbox{ where } 0<d(u,x)\le \epsilon \wedge 0<d(y,x) \leq \epsilon \mbox{ (*)} \nonumber
\eeqnarr
then $V^\prime$ is a gate-vertex set $V^\ast$. 
Furthermore, the smallest cardinality of set $V^\prime$ is equal to the smallest cardinality of gate-vertex set $V^\ast$: 
$min |V^\prime|=min |V^\ast|$. 
\ethm. 
\bproof
We will prove the condition (*) is a sufficient ($\Rightarrow$) and necessary ($Leftarrow$) condition for determining a gate-vertex set. 

\noindent{\bf ($\Rightarrow$):} If $V^\prime$ has this property, then we can iteratively recover the shortest-path distance through the consecutive local pairs. 
Based on the condition, for any non-local pair $u$ and $v$, we can discover $x_1 \neq u$ and $y_1 \neq v$ in $V^\prime$, such that $d(u,v)=d(u,x_1)+d(x_1,y_1)+d(y_1,v)$, where $d(u,x_1) \leq \epsilon$ and $d(y_1,v) \leq \epsilon$. 
If $d(x_1,y_1) \leq \epsilon$, then we find the sequence. 
If not, applying this condition for the non-local pair ($x_1,y_1$), we have $x_2 \neq x_1$ and $y_2 \neq y_1$ in $V^\prime$, such that 
$d(x_1,y_1)=d(x_1,x_2)+d(x_2,y_2)+d(y2,y_1)$ where $d(x_1,x_2) \leq \epsilon$ and $d(y_2,y_1) \leq \epsilon$. 
Clearly, if we can continue this process, eventually we have $d(x_i,y_i)\leq \epsilon$ (including the case where $x_i=y_i$) since the graph is finite. 
Thus, for any non-local pair $u$ and $v$, we can recover a sequence $(u,x_1,x_2, \cdots x_i,y_i, \cdots y_2,y_1,v)$, 
where each connective pair is a local pair. 
Thus, if a set $V^\prime$ has the property (*), then, it is a gate-vertex set. 

\noindent{\bf ($\Leftarrow$):} For any gate-vertex set $V^\ast$, it must have the property $(*)$. This can be immediately derived from the gate-vertex set definition.  

From the sufficient inference, we have $min |V^\prime| \leq min |V^\ast|$ and from the necessary inference, 
we have $min |V^\prime| \geq min|V^\ast|$.  Put together, we have $min |V^\prime|=min |V^\ast|$. 
\eproof

Based on Theorem~\ref{equivalent}, we introduce the following equivalent problem for discovering gate-vertex set. 

\bdefin({\bf Minimal Gate-Vertex Set Problem})
\label{gatevertexsetnew}
Given unweighted undirected graph $G=(V,E)$ and user-defined threshold $\epsilon$, we would like to discover a minimal set of vertices $V^\ast \subseteq V$ (gate-vertex sets) satisfing the following property: for any {\bf non-local pair} $u$ and $v$ ($d(u,v) > \epsilon$), there are vertices $x$ and $y$ in $V^\ast$, such that $d(u,x)+d(x,y)+d(y,v)=d(u,v)$, where $0<d(u,x)\leq \epsilon$ and $0<d(y,v) \leq \epsilon$. 
\edefin

\bthm({\bf NP-hardness of  Minimal Gate-Vertex Set Problem})
The minimal gate-vertex set problem is NP-hard. 
\ethm 
\bproof 
We can reduce the classical set cover problem (NP-hard) to this problem.
In the set cover problem, we have a ground set $U=\{u_1, u_2, \cdots, u_n\}$ which needs to be covered; and we have a list of candidate set $C_1, C_2, \cdots C_K$, which are subsets of $U$. We seek the minimal number of candidate sets to cover $U$, i.e.,$C_{i1} \cup C_{i2} \cup \cdots \cup C_{ik}=U$. 
Now, for the set cover instance, we build a tripartite graph $G=(X \cup C \cup Y, E)$, where $X=Y=U$ (each element in the ground set corresponds to a vertex in $X$ and a vertex in $Y$) , and each candidate set corresponding to a vertex in $C$. 
Then, if an element $u_i \in C_j$, then, $u_i$'s corresponding vertices in $X$ and $Y$ both link to $C_j$'s corresponding vertex in $C$. 
Given this, we claim that the minimal gate-vertex set with parameter $\epsilon=1$ corresponds the solution for  the minimal set cover problem. 
To observe this, we first can see that the vertices in the minimal gate-vertex set can only belong to $C$. 
If not, 

    
 
\eproof






\bdefin{\bf (Minimal Edges Discovery Problem)}
\label{edgediscovery}
Given an undirected graph $G=(V,E)$, the parameter $\epsilon$ and its corresponding gates $V^\ast$,
we want to find a set of weighted edges $E^\ast$ building the connections among $V^\ast$, and preserving the property:
\beqnarr
 d_G(u,v)= \nonumber \\
  min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon \wedge x,y \in V^\ast} (d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v)) \nonumber
\eeqnarr
where the number of edges $|E^\ast|$ is minimal.
\edefin

\comment{
The simplified graph is defined by using the vertex set $V^\ast$ and the edge set $E^\ast$.
To provide more flexibility, we also generalize our problem with exact distance preserving to the graph simplification problem with approximate distances.
Intuitively, more approximation error is allowed smaller the size of graph is.
By selecting suitable approximation ratio, users can adjust the trade-off between the simplicity of resulting graph and the accuracy of shortest distances.

\bdefin{\bf (Graph Simplification Problem with Approximate Distance)}
\label{agsprobdef}
Given an undirected graph $G=(V,E)$, the parameter $\epsilon$ and $\delta$,
its simplified graph $G^\ast=(V^\ast, E^\ast, W)$ ($V^\ast \subseteq V$)is an undirected weighted graph maintains following properties:

\noindent 1) $d_{G^\ast}(u,v) \le (1+\delta) d_G(u,v)$;

\noindent 2) $min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon} (d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v)) \le (1+\delta) d_G(u,v)$;

where both the number of vertices $|V^\ast|$ and the number of edges $|E^\ast|$ are minimal.
\edefin


\bdefin{\bf (Gates Discovery Problem)}
\label{agatediscovery}
Given an undirected graph $G=(V,E)$ and the parameter $\epsilon$, its corresponding gates are a subset of vertices $V^\ast \subseteq V$ keeping the following property:
\beqnarr
  min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon \wedge x,y \in V^\ast} (d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v)) \nonumber \\
  \le (1+\delta) d_G(u,v) \nonumber
\eeqnarr
where the number of gates $|V^\ast|$ is minimal.
\edefin

\bdefin{\bf (Minimal Edges Discovery Problem)}
\label{aedgediscovery}
Given an undirected graph $G=(V,E)$, the parameter $\epsilon$ and its corresponding gates $V^\ast$,
we want to find a set of weighted edges $E^\ast$ building the connections among $V^\ast$, and preserving the property:
\beqnarr
  min_{d_G(u,x) \le \epsilon \wedge d_G(y,v) \le \epsilon \wedge x,y \in V^\ast} (d_G(u,x) + d_{G^\ast}(x,y) + d_G(y,v)) \nonumber \\
  \le (1+\delta) d_G(u,v) \nonumber
\eeqnarr
where the number of edges $|E^\ast|$ is minimal.
\edefin
}

